Bijection: Parking-like structures and Tree-like structures

We recall the occupancy problem introduced by Konheim & Weiss in 1966 and we consider parking functions as hash maps. Each car $c_i$ prefers parking space $p_i$ (the hash map $c_i \mapsto p_i$ with $c_i$ is a key and $p_i$ an index into an array), if $p_i$ is occupied then $c_i$ the next available parking space (the hash table implementation using an open addressing strategy). This paper considers some others hash table implementations like hash tables with linked lists (with parking functions as hash maps). Using the Species Theory, we enumerate by Lagrange inversion those hash tables structures via a bijection with tree-like structures. This bijection provides a generalization of the Foata-Riordan bijection between parking functions and (forests of) rooted trees. Finally we show the number of hash tables with linked lists on a set of keys of cardinality $n$ is $n!C_n$, so the number of labeled binary trees with $n$ nodes.

==> autres.tex <==
\todo{blabla pour parler de tirage aléatoire}
%

The recursive definition (\ref{eq:pf_def_rec}) gives generating and enumerating
ways in terms of integer compositions (see \cite[Theorem 3.4]{priezvirmaux}).
Let $\pi := \pi_1\cdots \pi_k$ be a composition of the (non-negative) integer
$n$,
%
\begin{align*}
    \gf_\chi^\pi &= \binom{n}{\pi_1, \cdots, \pi_k}
                    \sum_{\tau\models \ell(\pi)}\prod_{i=1}^{\ell(\tau)}
                    \Psi_\tau(\chi; \pi, i) 
\intertext{wherein}
\Psi_\tau(\chi; \pi, i) &:= \begin{dcases*}
    \chi(1) & if $i = 1$,\\
    \chi(1 + \pi(\tau(i))) - \chi(1 + \pi(\tau(i-1))) & in otherwise;
\end{dcases*} 
\end{align*}
with $\pi(j) = \pi_1 + \cdots + \pi_j$. The formula $\gf_\chi^\pi$ is
enumerating parking functions $(Q_i) := \zeta(f)$ such
that for the sequence of indices $1 \ieq j_1 < j_2 < \cdots < j_{k'} \ieq
\chi(n)$ of non-empty sets of $(Q_i)$, one has $k' = k$ and $\card Q_{j_i} =
\pi_i$, for any $1 \ieq i \ieq k$.
% 
\begin{ex}
    Some of the $90 (=\gf^{212}_{Id})$ parking functions $(Q_i)$ associated to
    $212$:
    \begin{align*}
    \left\{\begin{aligned}
        12 | 3 | 45 | \cdot | \cdot \,,
        12 | 3 | \cdot | 45 | \cdot \,,
        12 | \cdot | 3 | 45 | \cdot \,, %
        13 | 2 | 45 | \cdot | \cdot \,,
        13 | 2 | \cdot | 45 | \cdot \,,
        13 | \cdot | 2 | 45 | \cdot \,, %
        14 | 3 | 25 | \cdot | \cdot \,,
        14 | 3 | \cdot | 25 | \cdot \,,\\
        14 | \cdot | 3 | 25 | \cdot \,, %
        23 | 1 | 45 | \cdot | \cdot \,,
        23 | 1 | \cdot | 45 | \cdot \,,
        23 | \cdot | 1 | 45 | \cdot \,, %
        24 | 3 | 15 | \cdot | \cdot \,,
        24 | 3 | \cdot | 15 | \cdot \,,
        24 | \cdot | 3 | 15 | \cdot \,, \cdots\quad\;%
    \end{aligned}\right\}
    \end{align*}
    (with the parking functions $\boldsymbol{(}\{\alpha, \beta, \cdots\},
    \{\gamma, \cdots\}, \cdots\boldsymbol{)}$ are noted
    $\alpha\beta\cdots|\gamma\cdots|\cdots$.)
\end{ex}

This formula is (quasi-)immediate from the recursive definition
(\ref{eq:pf_def_rec}) but it is clearly a non-efficient when the length of $\pi$
is huge ($\Theta(2^{\ell(\pi)})$). By inclusion-exclusion one obtains an
efficient formula:
%
\begin{prop} Let $\pi := \pi_1 \cdots \pi_k$ be a composition of $n$.
    \begin{align*}
        \gf^{\pi}_\chi = \binom{n}{\pi_1, \cdots,\pi_{k}}\sum_{j =
        0}^{k-1} (-1)^{k-j-1}\,
            \binom{\chi\left(\pi(j)+1\right) - j}{k - j}\,
            \gf^{\pi_1 \cdots \pi_j}_{\chi}
    \end{align*}
    and $\gf^{()}_\chi = 1$ (with $()$ the unique composition of
    $0$).
\end{prop}
%
\begin{preuve}
    \todo{\ldots}
\end{preuve}

==> bij.tex <==
%
\newpage
%


==> hash_map.tex <==
Hash table structure is an efficient way to implement dictionaries.
In some hash table implementation, search an element has complexity $\Theta(n)$
as \emph{chained hash tables with linked lists}. This fact comes from the 
\emph{hash collisions}, that means different keys are assigned to the same
bucket by the hash function.
In \cite{konheim1966occupancy}, the authors describes a collection of hash maps
which assume the ``\emph{occupancy discipline}'': Consider a finite set $U$ of
$u$ keys and a table of $n$ cells $C_0, C_1, \cdots, C_{n-1}$.


==> pf.tex <==
In \cite{priezvirmaux}, the authors give a constructive definition of
(generalized) parking functions species $\PF_\chi$ by the recursive definition:
Let $\chi : \NN_{>0} \to \NN_{>0}$ be an increasing map, 
\begin{align}
    \PF_\chi &:= \left(\setSp^{\chi(1)}\right)_{0} + 
                 \sum_{n \seq 1} \left(\setSp^{\chi(1)}\right)_{n} \cdot
                                 \PF_{\rho_n}\,,
&&\text{with}\qquad
    \rho_n : m \longmapsto \chi(n + m) - \chi(1)\,,
    %\label{eq:pf_def_rec} 
\end{align}
with $\setSp^{k}$ denotes the exponentiation of set species: $\setSp^k :=
\setSp \cdot \setSp^{k-1}$. In other terms, $\setSp^k$ is the species of
sequences of $k$-sets.
The notation $+$ is the sum of species and $(\setSp^k)_n$ is the restriction of
the species $\setSp^k$ to sets of cardinal $n$. (The readers may refer to
\cite{bergeron1998combinatorial} about Species theory, and to
\cite{priezvirmaux, stanley2002polytope, kung2003goncarov} about generalized
parking functions.)
%
\begin{prop}[\expandafter{\cite[Remark 2.1]{priezvirmaux}}]
    The parking functions species $\PF$ is isomorphic to the generalized parking
    functions species $\PF_{Id}$ (with $Id$ the identity map).
\end{prop}
%
\begin{preuve} 
    The map $\zeta : \pf \mapsto \left(\pf^{-1}(\{i\})\right)_{i \in
    \NN_{>0}}$ is a bijection between $\PF$-structures and
    $\PF_{Id}$-structures (and it commutes with the \textit{transport} (not
    defined there)).
\end{preuve}
%
\begin{remarq}
    In terms of hash map, each set $Q_i$ is the set of \emph{hash collisions} of
    keys that are assigned to the same bucket $i$.
\end{remarq}
%
\begin{ex}
    The first parking functions on the finite sets $[0],[1], [2]$ and $[3]$
    (with $[n] = \{1, \cdots, n\}$):
    \begin{align*}
    \PF[0] &= \left\{()\right\}\,;\quad \PF[1] = \left\{(1)\right\}\,; \quad
    \PF[2] = \left\{(12\mid\cdot),\; (1\mid2),\, (2\mid1)\right\}\,;\\
    \PF[3] &= \left\{\begin{array}{c}
        (123\mid\cdot\mid\cdot),\; (12\mid3\mid\cdot),\; (12\mid\cdot\mid3),\;
        (1\mid23\mid\cdot),\; (1\mid2\mid3),\; (1\mid3\mid2),\;
        (13\mid2\mid\cdot),\; (13\mid\cdot\mid 2),\\
        (23\mid1\mid\cdot),\; (23\mid\cdot\mid 1),\;
        (2\mid13\mid\cdot),\; (2\mid1\mid3),\; (2\mid3\mid1),\;
        (3\mid12\mid\cdot),\; (3\mid1\mid2),\; (3\mid2\mid1)
    \end{array} \right\}\,.
    \end{align*}
\end{ex}
%
\begin{remarq}
    From (\ref{eq:pf_def_rec}) a parking function $(Q_i)$ on a finite set of
    cardinal $n$ is a sequence of $n+1$-sets with $Q_{n+1} = \emptyset$. 
%     In the
%     sequel we represent a parking function on a finite set of cardinal $n$ as a
%     sequence of only $n$ sets.
\end{remarq}
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\subsection{Bijection with forest of rooted trees ($\F$-structures)}
    \label{ssec:bij_forest_rooted_trees}
%%%%%%%%%%%%%
%%%%%%%%%%%%%
In this subsection, we present (an adaptation of) the bijection of
\cite{foata1974mappings} with forest of rooted trees.
Let $(Q_i)$ be a parking function on $U$ (of cardinal $n$).
The following algorithm associates to $(Q_i)$ a forest of rooted trees on
$U$:
\begin{itemize}
  \item suppose a fixed order on $U$,
  \item set $<_q$ be a total order defined from $(Q_i)$:
  \begin{align*}
    u <_q u' \qquad \Longleftrightarrow \qquad \begin{dcases*}
        u < u' & if exists $j$ such that $u, u' \in Q_j$,\\
        j < k & with $u \in Q_j$ and $u' \in Q_k$.  
    \end{dcases*}
  \end{align*}
  \item set $Q_1$ be the root,
  \item following the order $u_1 <_q u_2 <_q \cdots <_q u_n$, set vertex 
    $u_i \to Q_{i+1}$, for each $u_i \in U$.
\end{itemize}
%
\begin{remarq}
    A $(Q_i)$ parking function on $U$ (of cardinal $u$) as defined by
    (\ref{eq:pf_def_rec}) is a sequence of $u+1$-sets (with $Q_{u+1}$ is empty).
\end{remarq}
%
\ \\[-20pt]
\begin{minipage}[c]{.66\linewidth}
    \color{fontcolor}
\begin{ex}
    \label{ex:bij_pf_rooted_trees_set_trees}
  Let $(23\mid \cdot \mid 5 \mid 16 \mid \cdot \mid 4\mid \cdot)$ be a parking
  function on $[6]$. 
  We associate the order $2<_q 3 <_q 5 <_q 1 <_q 6 <_q 4$ from the parking
  function (using the natural order on $[6]$).
  The forest of $\F[6]$ associated by the construction is:
\end{ex}
\end{minipage} \hfill
\begin{minipage}[c]{.36\linewidth}
\begin{align*}
\scalebox{.7}{\newcommand{\nna}{\node (a) {$2$};}%
\newcommand{\nnb}{\node (b) {$3$};}%
\newcommand{\nnc}{\node (c) {$5$};}%
\newcommand{\nnd}{\node (d) {$1$};}%
\newcommand{\nne}{\node (e) {$6$};}%
\newcommand{\nnea}{\node (ea) {$\emptyset$};}%
\newcommand{\nneb}{\node (eb) {$\emptyset$};}%
\newcommand{\nnec}{\node (ec) {$4$};}%
\newcommand{\nned}{\node (ed) {$\emptyset$};}%
\begin{tikzpicture}[auto]
\matrix[ampersand replacement=\&, column sep=.75cm, row sep=.2cm]{
%       \& \nna \& \nnb \\ 
% \nnea \&      \&      \& \nnc\\
%       \&      \&      \& \nnd \& \nne \\
%       \&      \&      \& \nneb\& \nnec\\
  \nna \& \nnea \\
  \nnb \& \nnc \& \nnd \& \nneb \\
       \&      \& \nne \& \nnec \& \nned\\
};
\node[draw,inner sep=2pt,ellipse,fit=(a) (b)] {};
\node[draw,inner sep=2pt,ellipse,fit=(c)](gc) {};
\node[draw,inner sep=2pt,ellipse,fit=(d) (e)] (gde) {};
\node[draw,inner sep=2pt,ellipse,fit=(ec)] (gec) {};
\path[thick] (a) edge (ea)
             (b) edge (gc)
             (c) edge (gde)
             (d) edge (eb) 
             (e) edge (gec)
             (ec) edge (ed);
\end{tikzpicture}}
\end{align*}
\end{minipage}
%\longleftrightarrow
% {\newcommand{\nna}{\node (a) {$2$};}%
% \newcommand{\nnb}{\node (b) {$3$};}%
% \newcommand{\nnc}{\node (c) {$5$};}%
% \newcommand{\nnd}{\node (d) {$1$};}%
% \newcommand{\nne}{\node (e) {$6$};}%
% \begin{tikzpicture}[auto]
% \matrix[ampersand replacement=\&, column sep=.1cm, row sep=.75cm]{
%       \& \node[circle, draw] (al) {$\alpha$};\\
%  \nna \&      \&\nnb \\ 
%       \&      \& \nnc\\
%       \& \nnd \&      \& \nne \\
% };
% \path[thick] (al) edge (a) edge (b)
%              (b) edge (c)
%              (c) edge (d) edge (e);
% \end{tikzpicture}}
%
Considering a fixed order on $U$, this construction is obviously reversible.
Furthermore we will see this bijection is a special case of a more generic
bijection between parking like structures and tree like structures (\todo{donner
la section}).
%%%%%%%%%%%%%
%%%%%%%%%%%%%
\subsection{Parking like species}
%%%%%%%%%%%%%
%%%%%%%%%%%%%
The recursive definition (\ref{eq:pf_def_rec}) of parking functions $\PF_\chi$
defines a parking function as a sequence of sets. Following the idea of the
definition, it seems natural to remplace the set species $\setSp$ by some other
species $\SP$:
%
\begin{align}
    \shift{\SP}{\chi} &:= \left(\SP^{\chi(1)}\right)_{0} + 
                 \sum_{n \seq 1} \left(\SP^{\chi(1)}\right)_{n} \cdot
                                 \shift{\SP}{\rho_n}\,.
    %\label{eq:def_shift}
\end{align}
%
We call the \emph{parking like species} over the
species $\SP$ the species $\shift{\SP}{\chi}$. (So one has $\PF_\chi =
\shift{\setSp}{\chi}$ and $\PF = \shift{\setSp}{Id}$.)
%
\begin{ex}
    Let $\linSp$ be the linear order species (defined by $\linSp = \oneSp +
    \singSp \cdot \linSp$ with $\oneSp$ is neutral species (such that
    $\oneSp[U] = \{U\}$ \textit{iff} $U = \emptyset$)). The
    $\shift{\linSp}{Id}$-structures on $[0], [1], [2]$ and $[3]$ are:
    \begin{align*}
    \shift{\linSp}{Id}[0] &= \left\{()\right\}\,; \quad
    \shift{\linSp}{Id}[1] = \left\{(1)\right\}\,; \quad
    \shift{\linSp}{Id}[2] = \left\{(12\mid\cdot),\; (21\mid\cdot),\;
                                   (1\mid2),\; (2\mid1)
    \right\}\,;\\
    \shift{\linSp}{Id}[3] &= \left\{\begin{array}{c}
        (123\mid \cdot\mid \cdot),\;
        (132\mid \cdot\mid \cdot),\;
        (213\mid \cdot\mid \cdot),\;
        (231\mid \cdot\mid \cdot),\;
        (312\mid \cdot\mid \cdot),\;
        (321\mid \cdot\mid \cdot),\\
        (12\mid 3\mid \cdot),\;
        (21\mid 3\mid \cdot),\;
        (12\mid \cdot \mid 3),\;
        (21\mid \cdot \mid 3),\;
        (13\mid 2\mid \cdot),\;
        (31\mid 2\mid \cdot),\\
        (13\mid \cdot \mid 2),\;
        (31\mid \cdot \mid 2),\;
        (23\mid 1\mid \cdot),\;
        (32\mid 1\mid \cdot),\;
        (23\mid \cdot \mid 1),\;
        (32\mid \cdot \mid 1),\\
        (1\mid 23 \mid \cdot),\;
        (1\mid 32 \mid \cdot),\;
        (2\mid 13 \mid \cdot),\;
        (2\mid 31 \mid \cdot),\;
        (3\mid 12 \mid \cdot),\;
        (3\mid 21 \mid \cdot),\\
        (1\mid 2 \mid 3),\;
        (2\mid 1 \mid 3),\;
        (1\mid 3 \mid 2),\;
        (3\mid 1 \mid 2),\;
        (2\mid 3 \mid 1),\;
        (3\mid 2 \mid 1)
    \end{array}
    \right\}\,.
    \end{align*}
\end{ex}
%
In terms of hashing this new species defines a concrete implementation
of ``\textit{hash table}''. For example if we considere $\SP := \linSp$ the
linear order species, the structures of species $\shift{\linSp}{Id}$ on a set of
keys $U$ are all possible \emph{chained hash tables with linked lists} using
parking functions as hash maps.

